Potentials of stable processes

For a stable process, we give an explicit formula for the potential measure of the process killed outside a bounded interval and the joint law of the overshoot, undershoot and undershoot from the maximum at exit from a bounded interval. We obtain the equivalent quantities for a stable process reflected in its infimum. The results are obtained by exploiting a simple connection with the Lamperti representation and exit problems of stable processes.

==> stable-defs.tex <==
\newcommand{\xiLS}{\xi^{\mathrm{L}}}
\newcommand{\xiCPP}{\xi^{\mathrm{C}}}
\newcommand{\CE}{\Psi}
\newcommand{\CELS}{\CE^{\mathrm{L}}}
\newcommand{\CECPP}{\CE^{\mathrm{C}}}
\newcommand{\LM}{\Pi}
\newcommand{\LMCPP}{\Pi^{\mathrm{C}}}
\newcommand{\LMLS}{\Pi^{\mathrm{L}}}
\newcommand{\LD}{\pi}
\newcommand{\LDCPP}{\pi^{\mathrm{C}}}
\newcommand{\LDLS}{\pi^{\mathrm{L}}}

% probability and expectation operators for the STABLE processes
\newcommand{\stP}{\mathrm{P}}
\newcommand{\stPh}{\mathrm{\hat P}}
\newcommand{\stE}{\mathrm{E}}
\newcommand{\stEh}{\mathrm{\hat E}}

% conditioned to stay positive
\newcommand{\stPup}{\stP^\uparrow}
\newcommand{\stEup}{\stE^\uparrow}
\newcommand{\hup}{h^\uparrow}
\newcommand{\LevPup}{\LevP^\uparrow}
\newcommand{\LevEup}{\LevE^\uparrow}

% conditioned to hit zero continuously
% include stmaryrd to get \ssearrow if desired
\ifdefined\ssearrow%
  \newcommand{\czcarrow}{\ssearrow} % \ssearrow is from stmaryrd
\else%
  \newcommand{\czcarrow}{\downarrow}
\fi
\newcommand{\stPdn}{\stP^\czcarrow}
\newcommand{\stEdn}{\stE^\czcarrow}
\newcommand{\hdn}{h^\czcarrow}
\newcommand{\LevPdn}{\LevP^\czcarrow}
\newcommand{\LevEdn}{\LevE^\czcarrow}
\newcommand{\Udn}{U^\czcarrow}
\newcommand{\udn}{u^\czcarrow}

% Lamperti processes
\newcommand{\xiup}{\xi^\uparrow}
\newcommand{\xidn}{\xi^\czcarrow}

\newcommand{\Xk}{X^*}
\newcommand{\stPk}{\mathrm{P}^*}
%\newcommand{\stPhk}{\mathrm{\hat P}^*}
\newcommand{\stEk}{\mathrm{E}^*}
%\newcommand{\stEhk}{\mathrm{\hat E}^*}

\newcommand{\Xh}{\hat{X}}
\newcommand{\Xsu}{\overline{X}}
\newcommand{\Xin}{\underline{X}}
\newcommand{\Xhsu}{\overline{\hat{X}}}
\newcommand{\Xhin}{\underline{\hat{X}}}

\newcommand{\LevP}{\mathbb{P}}
\newcommand{\LevE}{\mathbb{E}}
\newcommand{\LevPh}{\mathbb{\hat P}}
\newcommand{\LevEh}{\mathbb{\hat E}}
\newcommand{\LevPk}{\mathbb{P}^*}
\newcommand{\LevEk}{\mathbb{E}^*}
\newcommand{\xik}{\xi^*}
\newcommand{\xih}{\hat{\xi}}
\newcommand{\xihs}{\overline{\hat{\xi}}}
\newcommand{\xihi}{\underline{\hat{\xi}}}
\newcommand{\xis}{\overline{\xi}}
\newcommand{\xii}{\underline{\xi}}

% likewise for STABLE CONDITIONED TO AVOID ZERO
\newcommand{\stPaz}{\stP^\updownarrow}
\newcommand{\stPhaz}{\stPh^\updownarrow}
\newcommand{\Xaz}{X^\updownarrow}
\newcommand{\stEaz}{\stE^\updownarrow}
\newcommand{\stEhaz}{\stEh^\updownarrow}

% WEIRD SPED-UP LAMPERTI REPR of the STABLE PROCESS
\newcommand{\LevPp}{\LevP^\prime}
\newcommand{\LevEp}{\LevE^\prime}
\newcommand{\CEp}{\CE^\prime}
\newcommand{\xip}{\xi^\prime}

% WEIRD SPED-UP LAMPERTI REPR of stable CONDITIONED TO STAY POSITIVE
\newcommand{\Raz}{R^\updownarrow}
\newcommand{\xiaz}{\xi^\updownarrow}
\newcommand{\LevPaz}{\LevP^\updownarrow}
\newcommand{\LevEaz}{\LevE^\updownarrow}
\newcommand{\CEaz}{\CE^\updownarrow}


